Linearized Optimal Transport pyLOT Library: A Toolkit for Machine Learning on Point Clouds

The pyLOT library offers a Python implementation of linearized optimal transport (LOT) techniques and methods to use in downstream tasks. The pipeline embeds probability distributions into a Hilbert space via the Optimal Transport maps from a fixed reference distribution, and this linearization allows downstream tasks to be completed using off the shelf (linear) machine learning algorithms. We provide a case study of performing ML on 3D scans of lemur teeth, where the original questions of classification, clustering, dimension reduction, and data generation reduce to simple linear operations performed on the LOT embedded representations.

==> code_snippets.tex <==
The necessary libraries needed for running pyLOT on the tooth dataset and actually loading the tooth dataset are given by Listing \ref{code:imports}.

\begin{lstlisting}[language=Python, caption=Import Statements, label={code:imports}]
# Import necessary libraries
from pyLOT.classifier import LOTClassifier
from pyLOT.barycenters import LOTBarycenter
from pyLOT.embed import LOTEmbedding
from pyLOT.reduction import LOTDimensionalityReduction

# libraries for computation and plotting
import numpy as np
import matplotlib.pyplot as plt
from mpl_toolkits.mplot3d import Axes3D
from matplotlib.colors import ListedColormap
# libraries for PCA visualization
from sklearn.decomposition import PCA
# oversampling and train/test splits
from imblearn.over_sampling import RandomOverSampler
from sklearn.model_selection import train_test_split
# import time for timing how long code takes to run
import time
from datetime import datetime

ROOT_DIR = '../cleaned_real_data/'
SUB_DIR = ['Microcebus/','Mirza/','Saimiri/','Tarsius/']


def read_off(filepath):
    file = open(filepath)
    if 'OFF' != file.readline().strip():
        raise('Not a valid OFF File')
    n_verts, n_faces, n_edges = tuple([int(s) for s in file.readline().strip().split(' ')])
    verts = [[float(s) for s in file.readline().strip().split(' ')] for _ in range(n_verts)]
    return np.array(verts)
    
def load_data():
    # store file paths and tooth labels
    fp_lst = []
    xt_lst = []
    T_labels = []
    for dir in SUB_DIR:
        fps = os.listdir(ROOT_DIR + dir)
        fp_lst.extend(fps)
        T_labels.extend([dir[:-1]] * len(fps))

    for i in range(len(fp_lst)):
        xt = read_off(ROOT_DIR + T_labels[i] + '/' + fp_lst[i])
        xt_lst.append(xt)

    xt_lst = np.array(xt_lst)
    T_labels = np.array(T_labels)
    return xt_lst, T_labels

\end{lstlisting}

















 This associated code is in Listing \ref{code:lotEmbed}.

\begin{lstlisting}[language=Python, caption=Code to embed tooth samples., label={code:lotEmbed}]
xt_list, T_labels = load_fps() # load tooth dataset with appropriate labels
xr = np.random.normal(0, 1, size=(5000, 3)) # set reference measure with 5000 points

print('Generating Sinkhorn embeddings for tooth data...')
start_time = time.time()
# Compute LOT Sinkhorn embeddings with small lambda
T_embeddings_sh = LOTEmbedding.embed_point_clouds(xr, 
                                            xt_list,
                                            xt_masses=None, # allows masses if needed.  Defaults to None (i.e. assume uniform mass)
                                            sinkhorn=True, 
                                            lambd=0.05)
time_taken = time.time() - start_time
print(f'Time taken for Sinkhorn embeddings: {time_taken:.2f} seconds')

print('Generating LP embeddings for tooth data...')
start_time = time.time()
# Compute LOT embeddings
T_embeddings = LOTEmbedding.embed_point_clouds(xr, 
                                            xt_list,
                                            sinkhorn=False)
time_taken = time.time() - start_time
print(f'Time taken for LP embeddings: {time_taken:.2f} seconds')

print('Generating embeddings for tooth data with iterated embeddings...')
start_time = time.time()
all_bary_embeddings, \
    all_emd_lists, \
    barycenter_list, \
    barycenter_label_list = LOTEmbedding.compute_barycenter_embeddings(n_iterations=3, 
                                        embeddings=None, # starts from Gaussian reference if None, else generates barycenter from embeddings 
                                        labels=T_labels, # to generate class-specific barycenters 
                                        pclouds=xt_list, 
                                        masses=None, 
                                        n_reference_points=5000,
                                        n_dim=3 # dimension of data
                                        )
time_taken = time.time() - start_time
print(f'Time taken for iterated LP embeddings: {time_taken:.2f} seconds')

\end{lstlisting}




 The code to reproduce the tests here are given in Listing \ref{code:reduction}

\begin{lstlisting}[language=Python, caption=Code for PCA and LDA reduction., label={code:reduction}]
# run LDA for T_embeddings
T_lda, labels_balanced = LOTDimensionalityReduction.lda_reduction(T_embeddings, T_labels, n_components=3)
# plot 2D LDA
df_lda = pd.DataFrame(T_lda)
df_lda['label'] = label_balanced
fig = plt.figure(figsize=(8,6))
ax = sns.scatterplot(df_lda, x=0, y=1, hue='label')
sns.move_legend(ax, "lower center", bbox_to_anchor=(.7, 1), ncol=4, title=None, frameon=False)
plt.title("LDA CLuster (2D)", loc='left')
plt.savefig('../fig/cluster/gaussian_ref/lda_cluster_2d.png')
# plot 3D LDA
fig = plt.figure(figsize=(8,6))
ax = fig.add_subplot(1, 1, 1, projection='3d')
for l in df_lda['label'].unique():
    ax.scatter(df_lda[0][df_lda['label']==l], df_lda[1][df_lda['label']==l], df_lda[2][df_lda['label']==l],label=l)
ax.legend()
sns.move_legend(ax, "lower center", bbox_to_anchor=(.8, 1), ncol=4, title=None, frameon=False)
plt.title("LDA CLuster (3D)", loc='left')
plt.savefig('../fig/cluster/gaussian_ref/lda_cluster_3d.png')


# run PCA for T_embeddings
U, S, Vh, labels_balanced = LOTDimensionalityReduction.pca_reduction(T_embeddings, T_labels)
# plot 2D PCA
df_pca = pd.DataFrame(U)
df_pca['label'] = label_balanced
fig = plt.figure(figsize=(8,6))
ax = sns.scatterplot(df_pca, x=0, y=1, hue='label')
sns.move_legend(ax, "lower center", bbox_to_anchor=(.7, 1), ncol=4, title=None, frameon=False)
plt.title("PCA CLuster (2D)", loc='left')
plt.savefig('../fig/cluster/gaussian_ref/pca_cluster_2d.png')
# plot 3D PCA
fig = plt.figure(figsize=(8,6))
ax = fig.add_subplot(1, 1, 1, projection='3d')
for l in df_pca['label'].unique():
    ax.scatter(df_pca[0][df_pca['label']==l], df_pca[1][df_pca['label']==l], df_pca[2][df_pca['label']==l],label=l)
ax.legend()
sns.move_legend(ax, "lower center", bbox_to_anchor=(.8, 1), ncol=4, title=None, frameon=False)
plt.title("PCA CLuster (3D)", loc='left')
plt.savefig('../fig/cluster/gaussian_ref/pca_cluster_3d.png')

\end{lstlisting}



The code associated with the random oversampling is 

\begin{lstlisting}[language=Python, caption=Code for classification of teeth., label={code:classify}]
# generate train/test split and oversample
sampler = RandomOverSampler()
T_train, T_test, y_train, y_test = train_test_split(T_embeddings, T_labels, test_size=0.2, random_state=21)
# Keep 25 percent from each label OR oversampling (no duplicate on train and test)
X_train, y_train = sampler.fit_resample(T_train, y_train)
X_test, y_test = sampler.fit_resample(T_test, y_test)

# Train the classifier on the data
best_clf = LOTClassifier.get_best_classifier(X_train, y_train, X_test, y_test)
print("Best Classifier:\n", best_clf)
\end{lstlisting}




The results were generated by the following code:
\begin{lstlisting}[language=Python, caption=Code for barycenter generation., label={code:barycenter}]
# following code works for general situation but for specific case, assume that T_embeddings has only 3 samples per class (the ones from the visual)

# fixed weights for the three teeth
WEIGHTS_FIXED = np.array([
    [1,0,0], [0,1,0], [0,0,1], 
    [0.9, 0.1, 0], [0.9, 0, 0.1], [0.1, 0.9, 0], 
    [0, 0.9, 0.1], [0.1, 0, 0.9], [0, 0.1, 0.9],
    [0.6, 0.2, 0.2], [0.6, 0.3, 0.1], [0.6, 0, 0.4], 
    [0.2, 0.6, 0.2], [0.3, 0.6, 0.1], [0, 0.6, 0.4], 
    [0.2, 0.2, 0.6], [0.3, 0.1, 0.6], [0, 0.4, 0.6], 
    [0.2, 0.4, 0.4], [0.4, 0.2, 0.4], [0.4, 0.4, 0.2]
])

FIXED_SAMPLE_SIZE = 3
WEIGHTS_RAND_LEN = 20

WEIGHTS_RAND, R_labels = generate_weight(T_embeddings, T_labels, n=WEIGHTS_RAND_LEN)

tic = time.time()
# generate LOT barycenters with fixed weights for teeth in class
G_matrix, G_labels, _ = LOTBarycenter.generate_barycenters_within_class(T_embeddings, T_labels, WEIGHTS_FIXED, uniform=False, n=WEIGHTS_RAND_LEN)
toc = time.time()
print('Time taken for fixed-weights LOT barycenter', toc-tic)

# generate LOT barycenters with random weights for teeth in class
R_matrix, R_labels, WEIGHTS_RAND = LOTBarycenter.generate_barycenters_within_class(T_embeddings, T_labels, None, uniform=True, n=WEIGHTS_RAND_LEN)

# TRUE Barycenter calculations 
def compute_barycenter(xr, xt_class, w):
    b = np.ones((5000,)) / 5000
    measures_weights = [ot.unif(xt.shape[0]) for xt in xt_class]
    center = ot.lp.free_support_barycenter(xt_class, measures_weights, xr, b, w)

    return center

# Fixed Weights true barycenter
tic = time.time()
for label in np.unique(T_labels):
    print(datetime.now())
    C_matrix = []
    xt_class = xt_lst[T_labels == label][:FIXED_SAMPLE_SIZE]
    for weight in FIXED_WEIGHTS:
        C_matrix.append(compute_barycenter(xr, xt_class, weight))
    print(f"Generation for class {label} is done. (Fixed Weight)")
    with open(f'../pickle/C_matrix_{label}.pkl', 'wb') as file:
        file.write(pickle.dumps(np.array(C_matrix))) 
toc = time.time()
print('Time taken for fixed-weights true barycenter', toc-tic)

# Random Weights true barycenter
tic = time.time()
for label in np.unique(T_labels):
    print(datetime.now())
    B_matrix = []
    xt_class = xt_lst[T_labels == label]
    class_weight = WEIGHTS_RAND[R_labels == label]
    for weight in class_weight:
        B_matrix.append(compute_barycenter(xr, xt_class, weight))
    print(f"Generation for class {label} is done. (Random Weight)")
    with open(f'../pickle/B_matrix_{label}.pkl', 'wb') as file:
        file.write(pickle.dumps(np.array(B_matrix))) 
toc = time.time()
print('Time taken for random weights true barycenter', toc-tic)

# PLOTTING
Tarsius_0 = T_matrix[-33].reshape((5000,3))
Tarsius_1 = T_matrix[-32].reshape((5000,3))
Tarsius_2 = T_matrix[-31].reshape((5000,3))

# Plot sample 1
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(Tarsius_0[:,0], Tarsius_0[:,1], Tarsius_0[:,2], c = Tarsius_0[:,2])
plt.title("Tooth Sample #1")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/tarsius_first.png')

# Plot sample 2
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(Tarsius_1[:,0], Tarsius_1[:,1], Tarsius_1[:,2], c = Tarsius_1[:,2])
plt.title("Tooth Sample #2")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/tarsius_second.png')

# Plot sample 3
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(Tarsius_2[:,0], Tarsius_2[:,1], Tarsius_2[:,2], c = Tarsius_2[:,2])
plt.title("Tooth Sample #3")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/tarsius_third.png')

# Plot LOT Barycenter using tooth sample 1 and 3
G = G_matrix[-10].reshape((5000,3))
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(G[:,0], G[:,1], G[:,2], c = G[:,2])
plt.title("LOT Approx. Barycenter using #1 & #3")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/Tarsius_AB_13.png')

# Plot LOT Barycenter using tooth sample 2 and 3
G = G_matrix[-7].reshape((5000,3))
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(G[:,0], G[:,1], G[:,2], c = G[:,2])
plt.title("LOT Approx. Barycenter using #2 & #3")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/Tarsius_AB_23.png')

# Plot True Barycenter using tooth sample 1 and 3
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(C_matrix_Tarsius[-10][:,0], C_matrix_Tarsius[-10][:,1], C_matrix_Tarsius[-10][:,2], c = C_matrix_Tarsius[-10][:,2])
plt.title("True Barycenter using #1 & #3")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/Tarsius_TB_13.png')

# Plot True Barycenter using tooth sample 2 and 3
fig = plt.figure()
ax = fig.add_subplot(1, 1, 1, projection='3d')
ax.scatter(C_matrix_Tarsius[-7][:,0], C_matrix_Tarsius[-7][:,1], C_matrix_Tarsius[-7][:,2], c = C_matrix_Tarsius[-7][:,2])
plt.title("True Barycenter using #2 & #3")
plt.savefig('../fig/barycenter_comp/fixed_weight_example/Tarsius_TB_23.png')


\end{lstlisting}





With code applied to the tooth dataset, we simply run \texttt{LOTEmbedding.compute\_barycenter\_embeddings} and plot.  In particular, we have the following code:
\begin{lstlisting}[language=Python, caption=Code for iterative barycenter generation., label={code:iterBary}]
all_bary_embeddings, \
    all_emd_lists, \
    barycenter_list, \
    barycenter_label_list = LOTEmbedding.compute_barycenter_embeddings(n_iterations=3, 
                                        embeddings=None,
                                        labels=T_labels, 
                                        pclouds=xt_list, 
                                        masses=None, 
                                        n_reference_points=5000,
                                        n_dim=3
                                        )
# all_bary_embeddings contain all the iterative embeddings with respect to the barycenters for each class
# barycenter_label_list contains barycenters after successive embeddings
# run similar plotting, dimensionality reduction, and classifier analysis as before
\end{lstlisting}



